Fusing Depthwise and Pointwise Convolutions for Efficient Inference on GPUs

Depthwise and pointwise convolutions have fewer parameters and perform fewer operations than standard convolutions. As a result, they have become increasingly used in various compact DNNs, including convolutional neural networks (CNNs) and vision transformers (ViTs). However, they have a lower compute-to-memory-access ratio than standard convolutions, making their memory accesses often the performance bottleneck. This paper explores fusing depthwise and pointwise convolutions to overcome the memory access bottleneck. The focus is on fusing these operators on GPUs. The prior art on GPU-based fusion suffers from one or more of the following: (1) fusing either a convolution with an element-wise or multiple non-convolutional operators, (2) not explicitly optimizing for memory accesses, (3) not supporting depthwise convolutions. This paper proposes Fused Convolutional Modules (FCMs), a set of novel fused depthwise and pointwise GPU kernels. FCMs significantly reduce pointwise and depthwise convolutions memory accesses, improving execution time and energy efficiency. To evaluate the trade-offs associated with fusion and determine which convolutions are beneficial to fuse and the optimal FCM parameters, we propose FusePlanner. FusePlanner consists of cost models to estimate the memory accesses of depthwise, pointwise, and FCM kernels given GPU characteristics. Our experiments on three GPUs using representative CNNs and ViTs demonstrate that FCMs save up to 83\% of the memory accesses and achieve speedups of up to 3.7x compared to cuDNN. Complete model implementations of various CNNs using our modules outperform TVMs' achieving speedups of up to 1.8x and saving up to two-thirds of the energy. FCM and FusePlanner implementations are open source: https://github.com/fqararyah/Fusing_DW_and_PW_on_GPUs.

==> sections/3_conv_data_movement.tex <==
\section{Convolution data movement on GPU}
\label{sec:conv_dm}

The FCMs target minimizing \emph{global memory access}, and data movement in general. We use the term global memory access to refer to accesses to both GPU's L2 and the global memory. Hence, in this section, we explore the design choices that govern data movement in a convolution implementation. We focus on the direct convolution implementation and use it as the basis for FCMs (Section~\ref{sec:fcms}) because other implementations including Winograde and FFT require filters with greater than $1 \times 1$ width and height and so are not applicable for PW convolution~\cite{lavin2016fast}. Moreover, both of them, as well as GEMM, optimize the computation at the cost of more memory BW requirements which is not suitable for the memory-bound convolutions. The main design choices governing data movement are (1) dataflow; (2) data layout, and (3) tiling. They affect both the layer-by-layer (LBL) implementation and the fused one similarly. Their impact in the context of the FCMs is highlighted throughout Sections~\ref{sec:fcms}, and ~\ref{sec:fuseestimator}. Note that by LBL we refer to the convolutional layers processing. We consider the cases where a convolution is fused with normalization and activation but not with another convolution as LBL.

% Moreover, PW convolutions have filters of $1 \times 1$ width and height, but FFT is beneficial for filters greater than $5 \times 5$, and Winograd is applicable when a filter width and height are greater than 1~\cite{lavin2016fast}.

 \begin{figure}[!htbp]
         \centering
         \captionsetup{justification=centering}
         \includegraphics[width=0.9\linewidth]{figures/conv_on_gpu.pdf}
         \caption{Simplified examples of OS dataflow of two mapping options of pointwise convolution on GPU}
         \label{fig:conv_on_gpu}
\end{figure}

\subsection{Dataflow}
\label{subsec:dataflow}
There are three common convolution dataflows, each minimizes global memory accesses in one of the three arrays processed by a convolutional layer, \textit{i.e.} weights, IFMs, and OFMs (and partial sums)~\cite{chen2016eyeriss}. The Weight Stationary dataflow (WS) minimizes weights' global memory accesses by keeping weights closest to the compute units (maximizing weight reuse). The Output Stationary (OS) minimizes partial sums' global memory accesses by keeping the accumulation closest to the compute units. The Input Stationary (IS) minimizes IFMs' global memory accesses. 

For each dataflow, there are several ways to map a convolution on a GPU, each having its own parallelism, and memory access cost and patterns. Figure~\ref{fig:conv_on_gpu} shows an example of two OS mapping variants of a PW convolution with four filters and $6 \times 6 \times 4$ IFMs on a GPU with two SMs. Note that this example is simplified, in practice both the weights and FMs should usually be partitioned to fit in the SMs resources and to maximize SMs utilization. In Mapping1, SM1 produces the first and second OFM channels, and SM2 produces the third and fourth. In Mapping2 SM1 produces the upper half of all OFMs channels and SM2 produces the lower half. 

Each of the two mappings has its own global memory access. Since each SM has its own L1/shared memory, in the first mapping the IFM elements are read twice, and the weights are partitioned. So, the overall weights and IFMs global memory access are $2 \times IFMs\ size + weights\ size$, which is $304$. On the other hand, in the second mapping, the weights are replicated and the IFMs are partitioned. So, the overall weights and IFMs global memory access are $2 \times weights\ size + IFMs\ size$, resulting in $176$, which saves $42\%$ of the accesses compared to Mapping1. Note that, for simplicity, the example assumes that the shared memory is large enough and that the only misses in L1 are compulsory. 

Mapping has a direct impact on reuse as well. For example, considering weight reuse, since each filter slides over a whole channel in the IFMs and since Mapping1 assigns all FMs to each SM, a single weight could be loaded into a thread register and used $6 \times 6$ times. This means that $36$ MAC operations could be done using a single load of a weight. In Mapping2, the maximum achievable weight reuse is $18$. 
%Considering activation reuse, each activation is convolved with the four filters hence it can be loaded once and used four times. In mapping1, as two filters are assigned to each SM, the maximum achievable activation reuse is $2$. In mapping2, an activation reuse of $4$ could be achieved.

\subsection{Data layout}
\label{subsec:datalayout}
Data layout has a significant impact on the convolution performance~\cite{li2016optimizing}. The two commonly used data layouts by DL libraries are NCHW and NHWC, where N stands for Number of data samples, C for channels, H for height, and W for width. These layouts are also known as channels-first and channels-last, respectively. The combination of data layout and the data access patterns of an algorithm affects global memory access in two ways. \textbf{First}, the more scattered the addresses are, the less the throughput. For example, if the used convolution algorithm is parallelized on IFMs' channels only, then the threads in a warp access elements that are adjacent on the channel's dimension. In this case, NHWC is preferred as it guarantees that threads in a warp access contiguous memory locations. \textbf{Second}, GPU global memory is accessed via multiples of 32 byte-transactions (32, 64, or 128). When an instruction that accesses global memory is executed, the memory accesses of the threads within a warp are coalesced into one or more memory transactions. Memory transactions in which the first address is a multiple of the transaction size maximize memory throughput, such transactions are known as \emph{naturally aligned}.

\begin{figure}[!htbp]
         \centering
         \captionsetup{justification=centering}
         \includegraphics[width=0.9\linewidth]{figures/conv_tiling.pdf}
         \caption{Overlapped IFM tiles in depthwise convolution.}
         \label{fig:tiles_overlapping}
\end{figure}

\begin{equation}
\label{eq:tiles_overlapping}
\small
\begin{split}
\text{IFM overlap} = &(\ceil*{ \frac{\text{IFM width}}{\text{tile width}} } - 1) * (Fw - \text{strides}) *  \text{IFM height} \ \\
& + \\
&(\ceil*{\frac{\text{IFM height}}{\text{tile height}} } - 1) * (Fh - \text{strides}) * \text{IFM width}
\end{split}
\end{equation}

\subsection{Tiling}
\label{subsec:tiling}

On a GPU, each tile is given to a thread block and is processed by an SM. Figure~\ref{fig:tiles_overlapping} shows a simple 2-D example where a $3 \times 3$ OFM tile is produced using $5 \times 5$ IFM tile and a $3 \times 3$ filter. As the figure shows, IFM tiles do overlap. The values in the overlapping areas must be loaded redundantly. Hence, to minimize global memory access the tile sizes and shapes should be selected to minimize the overall overlapping. Equation~\ref{eq:tiles_overlapping} is used to calculate overlapping within an IFM where \emph{Fw} is filter width and \emph{Fh} is filter height. Note that in this equation, the intersection of the horizontal and vertical overlapping areas is calculated twice to keep it proportional to the number of memory accesses. For example, the four IFM elements at the intersection of the four tiles in Figure~\ref{fig:tiles_overlapping} are loaded four times, which is twice the number of times other overlapping area elements are loaded. As can be inferred from the equation and Figure~\ref{fig:tiles_overlapping}, the bigger the tiles the less overall overlapping. However, there is a limit on tile sizes. If \emph{shared memory} is used to store IFMs, OFMs, and weight tiles, then the summation of these three tile sizes must not exceed the size of the SM's shared memory. Even if \emph{shared memory} is not used to store all the tiles, tile sizes that exceed L1 cache may result in L1 misses which affects the performance. Tile shape also affects memory access. As the figure shows, the overlapping areas correspond to some sides of a tile perimeter. Since the rectangle with the smallest perimeter with a given area is a square, square tiles or tiles with close width and height result in less overlapping.
